Constructing Multi-Modal Dialogue Dataset by Replacing Text with Semantically Relevant Images

In multi-modal dialogue systems, it is important to allow the use of images as part of a multi-turn conversation. Training such dialogue systems generally requires a large-scale dataset consisting of multi-turn dialogues that involve images, but such datasets rarely exist. In response, this paper proposes a 45k multi-modal dialogue dataset created with minimal human intervention. Our method to create such a dataset consists of (1) preparing and pre-processing text dialogue datasets, (2) creating image-mixed dialogues by using a text-to-image replacement technique, and (3) employing a contextual-similarity-based filtering step to ensure the contextual coherence of the dataset. To evaluate the validity of our dataset, we devise a simple retrieval model for dialogue sentence prediction tasks. Automatic metrics and human evaluation results on such tasks show that our dataset can be effectively used as training data for multi-modal dialogue systems which require an understanding of images and text in a context-aware manner. Our dataset and generation code is available at https://github.com/shh1574/multi-modal-dialogue-dataset.

==> ___0.RelatedWork.tex <==
\section{Related Work}
\label{relatedwork}

\subsection{Vision and Launguage Tasks}
Image captioning is a representative task of generating text by understanding the context of an image. MS-COCO~\citep{lin2014microsoft} and Flickr30k~\citep{young2014image} datasets are mainly used for this task. This work is discussed largely with caption generation models based on a sequence-to-sequence model~\citep{xu2015show, vinyals2015show, you2016image, anderson2018bottom}, and retrieval-based models~\citep{nam2017dual, faghri2017vse, gu2018look}. Since captioning tasks are useful for understanding the relationship between text and images based on image-text pairs, we use image caption datasets for multi-modal conversation data construction and learning our model.

The image-text matching task is based on a measure of visual-semantic similarity between a text and an image. A typical solution is learning a common space to compare feature vectors of text and images. While various methods have been discussed in this area~\citep{frome2013devise, kiros2014unifying, vendrov2015order}, we consider recent studies focusing on improving a global image representation. \citet{li2019visual} proposed a reasoning model that generates a global image representation that captures the key objects and semantic concepts of the image. The model builds connections between image regions and performs inference over the Graph Convolutional Network~\citep{kipf2016semi} to generate semantic representation. We make a judgment that such work will help to find images suitable for dialogue sentences. We replace some sentences of the source text datasets with appropriate images using this model.

\subsection{Multi-modal Conversation}
The major researches on human conversation focus on text-based tasks. Most of the conversation datasets used in these tasks are text-only datasets~\citep{li2017dailydialog, rashkin2018towards, zhang2018personalizing}. Conversations are mainly in natural language, but people sometimes incorporate images into conversations. Thus, this research area extends to a multi-modal conversation.

There are visual question answering~\citep{antol2015vqa} or generation~\citep{mostafazadeh2016generating}, and visual dialogue~\citep{das2017visual}. They are one-sided QA exchanges that answer a single dialogue sentence to a factual question for an image. Due to the failure to consider the previous textual context, this work is far from natural human conversations.

\citet{mostafazadeh2017image} proposed a task about a pair of question and answer that considers the visual and textual context. They build validation and test datasets based on 4k images called Image Grounded Conversations (IGC). Although they do not provide training datasets, they contribute to present dialogue tasks based on visual and contextual inference. However, conversations of this task is also a limited situation with questions.

To extend the IGC task, \citet{shuster2020image} proposed a large-scale image-grounded conversation dataset, Image-Chat, collected through crowd-workers. Their dataset consists of 202k image-based conversations using 215 style characteristics. Since the conversations progress around a given image, the image is independently interpreted regardless of the context prior to the image. However, dialogues that will follow in the image used to answer or explain the question is affected by the previous context of the image. To include these situations, our work contains various image use cases of the human conversation. Furthermore, since the datasets collected by the crowd are sophisticated but transient, we consider a data building method that can be created automatically.


==> ___1.Models.tex <==
\section{Models}
\label{models}
% 모델 Figure 필요함.

Our goal is to handle an image as a part of a Multi-Modal Conversation, converting images into context-aware caption considering previous contexts, not just simple caption. To this end, two major dialogue models are used: retrieval and generative. Both models commonly use three different sub-network: (i) an image encoder, (ii) a text encoder, (iii) a fusion layer. Fusion layer combines encoded image representation and text representation, and this combined representation fed into  different modules depending on which dialogue model it is. In the retrieval model, the combined representation is used for calculating similarity with candidate responses. For the generation model, the combined representation fed into RNN-based Encoder-Decoder Model to generate context-aware caption word by word.

\subsection{Image Encoder}
% VSRN에 대한 간단한 설명
% 1. Bottom-up attention, 2. GCN, 3.Gobal semantic reasoning (VSRN 구조 그대로 차용)
% 일단 VSRN과 구조 똑같으니까 거기 쓰인 문장 고대로 가져옴. 나중에 Rephrase하면 될 듯
For the image encoder, all the image representations are generated by bottom-up attention model, and then encoder builds up connections between these image regions and do reasoning using Graph Convolutional Networks (GCN) to generate features with semantic relationship information. Up to this point, the shape of image representation is (36 x embed\_size), $r_{GCN}$. Then, we do global semantic reasoning on these relationship-enhanced features to select the discriminative information and filter out unimportant one to generate the final representation for the whole image, and the shape of the final representation, $r_I$, has embed\_size.
\subsection{Text Encoder}
For the context and context-aware dialogue representation, same text encoder is shared. Two major types of text encoder are used: RNN and BERT. 1-layer GRU is used as RNN-based Text encoder, and pretrained BERT-base as BERT-based Text encoder. The final representation of both context and context-aware dialogue, respectively $r_C$ and $r_D$, has embed\_size shape which is same as final image representation. In specific, the final representation of [CLS] token is used as final context representation\
The reason why we use pre-trained BERT model is that the more words model knows, the better model understands the context and context-aware dialogue. 

% Context, Target 모두 같은 Text encoder를 Share함
% 1. RNN
% 2. BERT : 사전 학습이 되지 않은 RNN을 사용하는 것보다, 각 단어의 의미를 어느정도 학습했고, 문장을 하나의 Representation으로 만들어내는 능력이 있는 BERT 사용
% CLS Token의 Representation이 각 Context와 Target dialog를 나타냄

\subsection{Fusion module}
To replace image to proper context-aware dialogue, combining the image and context representation into one fused representation, $r_F$, is important. We consider four possible fusion modules for the inputs:

% 아래 두 개는 수식 쓰기 애매한데 어떻게 해야되지
\textit{Summation}: Because both image and context representation have same shape, it is easy to add two representation. The final representation is computed as $r_F = r_I + r_C$.

\textit{Element-wise Product}: Similar to the Summation, two representations are multiplied by element-wise manner. The final representation is computed as $r_F = r_I \cdot r_C$.

\textit{Concatenation}: Simple summation and product may not capture the relevance of the image and context representation. To handle this, two representations are concatenated and fed into linear layer to make it the same size as context-aware dialogue representation.

\textit{Attention-based Fusion}: In most cases, the importance and relevance of each image and context vary for making combined representation for every instance. Thus, two representations are concatenated, and fed into 2-layers Transformer Encoder which performs self-attention over them.

% Image representaiton과 Context representation을 잘 융합해야 한다.
\subsection{Training and Inference}
\paragraph{Loss function}
% Retrieval -> Contrastive Loss
% Generative -> Caption generation loss

\paragraph{Pre-trained Image Encoder}
\paragraph{Two-step training strategies}
% Loss function -> combined representation과, Context represenation을 가깝게 만드는 loss

% Pre-training -> Image representation과, Object들의 관계를 배우기 위해, coco, flickr captioning으로 pretraining을 시킴.

% Two-step training -> 처음 보는 Context에 대해서도 잘 이해하기 위해서는 최대한 많은 대화를 보는 것이 필요함. 하지만 Pre-training에서는 caption들을 많이 봤기 때문에 더 많은 대화를 보여줄 필요가 있음. 우리 Multi-Modal Conversation dataset에서 하나의 전체 대화에 대해 하나의 문장만 이미지로 치환되는 특성상, Training에 쓰이는 Context + Image -> target dialog instance 외의 문장들은 전혀 학습에 쓰이지 않음. 따라서 Image 없이 context만 보고 다음 대화를 예측하게 하는 instance를 여러개 만들어서 추가로 학습 시키면, training 과정에서 우리 데이터셋에 있는 모든 문장을 모두 학습할 수 있게 됨.
% Main task로 넘어가기전에, 1 epoch

